Med-PMC: Medical Personalized Multi-modal Consultation with a Proactive Ask-First-Observe-Next Paradigm

The application of the Multi-modal Large Language Models (MLLMs) in medical clinical scenarios remains underexplored. Previous benchmarks only focus on the capacity of the MLLMs in medical visual question-answering (VQA) or report generation and fail to assess the performance of the MLLMs on complex clinical multi-modal tasks. In this paper, we propose a novel Medical Personalized Multi-modal Consultation (Med-PMC) paradigm to evaluate the clinical capacity of the MLLMs. Med-PMC builds a simulated clinical environment where the MLLMs are required to interact with a patient simulator to complete the multi-modal information-gathering and decision-making task. Specifically, the patient simulator is decorated with personalized actors to simulate diverse patients in real scenarios. We conduct extensive experiments to access 12 types of MLLMs, providing a comprehensive view of the MLLMs' clinical performance. We found that current MLLMs fail to gather multimodal information and show potential bias in the decision-making task when consulted with the personalized patient simulators. Further analysis demonstrates the effectiveness of Med-PMC, showing the potential to guide the development of robust and reliable clinical MLLMs. Code and data are available at https://github.com/LiuHC0428/Med-PMC.

==> table/auto.tex <==
\begin{table*}[ht]
\centering
% \setlength{\tabcolsep}{1mm}
\fontsize{9}{9}\selectfont{
\begin{tabular}{ccccc|c|ccc}
\toprule
\multirow{2}*{Model} &\multicolumn{4}{c|}{Overall Competency} &\multicolumn{1}{l|}{Multi-turn} &\multicolumn{3}{c}{Multi-modal} \\
 &Inquiry &Examination  &Diagnosis & Treatment &info\_gain &MMA &Contras-1 &Contras-2 \\ \midrule
\multirow{2}*{Mini-InternVL-1.5\shortcite{mini-internvl-1.5}}  &50.43 &10.29 &23.01&18.97 &3.40 &10.48 &46.25 &16.34 \\
\textcolor{red}{ }  &\textcolor{red}{ 39.44} &\textcolor{red}{ 15.02} &\textcolor{red}{ 22.07}&\textcolor{red}{ 19.89} &\textcolor{red}{ 3.80} &\textcolor{red}{ 9.33} &\textcolor{red}{ 43.14} &\textcolor{red}{ 14.01} \\ \midrule
\multirow{2}*{InternVL-1.5\shortcite{internvl-1.5}}  &52.42 &13.84 &26.32&21.44 &4.58 &13.94 &45.85 &17.16 \\
\textcolor{red}{ } &\textcolor{red}{ 42.91} &\textcolor{red}{ 7.33}  &\textcolor{red}{ 25.72}&\textcolor{red}{ 20.53} &\textcolor{red}{ 3.49} &\textcolor{red}{ 8.82} &\textcolor{red}{ 34.93} &\textcolor{red}{ 12.06} \\ \midrule
\multirow{2}*{Gemini-flash\shortcite{reid2024gemini}}  &63.99 &17.95 &37.81&26.75 &4.12 &19.25 &74.97 &30.47 \\
\textcolor{red}{ }  &\textcolor{red}{ 56.15} &\textcolor{red}{ 22.89} &\textcolor{red}{ 31.77}&\textcolor{red}{ 22.88} &\textcolor{red}{ 3.45} &\textcolor{red}{ 14.08} &\textcolor{red}{ 48.42} &\textcolor{red}{ 19.35} \\ \midrule
\multirow{2}*{Gemini-pro\shortcite{reid2024gemini}}  &68.19 &26.74&46.21&32.95 &4.55 &11.35 &62.12 &29.93 \\
\textcolor{red}{ }  &\textcolor{red}{ 61.04} &\textcolor{red}{ 23.89} &\textcolor{red}{ 37.66}&\textcolor{red}{ 28.64} &\textcolor{red}{ 3.3} &\textcolor{red}{ 8.89} &\textcolor{red}{ 52.67} &\textcolor{red}{ 24.8} \\ \midrule
\multirow{2}*{GLM4v\shortcite{glm2024chatglm}} &32.19 &10.73 &21.75 &19.97 &4.95 &25.06 &61.95 &15.39 \\
\textcolor{red}{ }  &\textcolor{red}{ 30.36} &\textcolor{red}{ 17.86} &\textcolor{red}{ 19.23}&\textcolor{red}{ 17.72} &\textcolor{red}{ 5.94} &\textcolor{red}{ 22.46} &\textcolor{red}{ 59.72} &\textcolor{red}{ 14.69} \\ \midrule
\multirow{2}*{GPT-4o\shortcite{GPT-4o}}  &68.75 &32.50 &45.12&32.25 &4.87&20.76 &58.71 &27.07 \\
\textcolor{red}{ }  &\textcolor{red}{ 61.33} &\textcolor{red}{ 29.62} &\textcolor{red}{ 44.32}&\textcolor{red}{ 28.66} &\textcolor{red}{ 4.29} &\textcolor{red}{ 17.29} &\textcolor{red}{ 55.42} &\textcolor{red}{ 25.00} \\ \midrule
\multirow{2}*{GPT-4o mini\shortcite{Mini-GPT-4o}}  &68.25	&25.20	&46.83	&32.17 &4.22 &6.45	&36.38	&4.79\\
\textcolor{red}{ }  &\textcolor{red}{ 60.99} &\textcolor{red}{ 21.34} &\textcolor{red}{ 37.94}&\textcolor{red}{ 26.41} &\textcolor{red}{ 3.67} &\textcolor{red}{ 3.30} &\textcolor{red}{ 24.50} &\textcolor{red}{ 3.49} \\ \midrule
\multirow{2}*{GPT-4v\shortcite{gpt4v}}  &68.28 &25.50 &44.17&32.19 &4.46 &20.59 &74.25 &34.36 \\
\textcolor{red}{ }  &\textcolor{red}{ 60.51} &\textcolor{red}{ 25.16} &\textcolor{red}{ 36.57}&\textcolor{red}{ 31.81} &\textcolor{red}{ 5.10} &\textcolor{red}{ 24.32} &\textcolor{red}{ 73.25} &\textcolor{red}{ 31.64} \\ \midrule
\multirow{2}*{Qwen-vl-chat-v1\shortcite{Qwen-VL-chat}}  &57.48 &15.06 &29.47&23.98 &5.01 &2.46 &23.86 &15.40 \\
\textcolor{red}{ }  &\textcolor{red}{ 48.28} &\textcolor{red}{ 11.58} &\textcolor{red}{ 25.06}&\textcolor{red}{ 22.98} &\textcolor{red}{ 5.24} &\textcolor{red}{ 2.77} &\textcolor{red}{ 22.04} &\textcolor{red}{ 12.09} \\ \midrule
\multirow{2}*{Qwen-vl-max\shortcite{Qwen-VL-max}} &56.34 &19.66 &28. 61&27.08 &4.68 &15.20 &63.43 &24.01 \\
\textcolor{red}{ } &\textcolor{red}{ 47.75} &\textcolor{red}{ 20.22} &\textcolor{red}{ 28.93} &\textcolor{red}{ 22.13} &\textcolor{red}{ 4.34} &\textcolor{red}{ 19.61} &\textcolor{red}{ 64.73} &\textcolor{red}{ 23.78} \\ \midrule
\multirow{2}*{HuatuoGPT-Vision-7B\shortcite{chen2024huatuogpt-vision}} &54.87 &10.95 &32.78&25.41 &3.11 &5.14 &16.47 &0.82 \\
\textcolor{red}{ } &\textcolor{red}{ 47.80} &\textcolor{red}{ 10.14} &\textcolor{red}{ 24.56} &\textcolor{red}{ 25.95} &\textcolor{red}{ 3.47} &\textcolor{red}{ 7.53} &\textcolor{red}{ 28.23} &\textcolor{red}{ 1.51} \\ \midrule
\multirow{2}*{HuatuoGPT-Vision-34B\shortcite{chen2024huatuogpt-vision}} &59.34 &24.52 &40.54&27.29 &4.04 &16.22 &46.67 &5.14 \\
\textcolor{red}{ } &\textcolor{red}{ 51.12} &\textcolor{red}{ 28.32} &\textcolor{red}{ 36.04} &\textcolor{red}{ 24.20} &\textcolor{red}{ 3.79} &\textcolor{red}{ 12.37} &\textcolor{red}{ 46.05} &\textcolor{red}{ 2.33} \\\bottomrule
\end{tabular}}
\caption{The auto-metric evaluation results about the standard patient and actor patient of different doctor models. The black denotes the result is evaluated with the standard patient and the red denotes with the actor patient. }
\label{tab:auto}
\end{table*}

==> table/auto_one_cot.tex <==
\begin{table*}[h]
\centering
\fontsize{9}{9}\selectfont{
\begin{tabular}{ccccc|c|ccc}
\toprule
\multirow{2}{*}{Model} &\multicolumn{4}{c|}{Overall Competency} &Multi-turn &\multicolumn{3}{c}{Multi-modal} \\
  &Inquiry &Examination  &Diagnosis & Treatment &info\_gain &MMA &Contras-1 &Contras-2 \\ \midrule
\multirow{2}{*}{Gemini-pro}  &54.11 &29.52 &44.39&28.62 & 4.31 &11.08 &52.23 &5.22 \\
 &\textcolor{red}{ 51.51} &\textcolor{red}{21.52}&\textcolor{red}{ 32.49} &\textcolor{red}{ 29.38} &\textcolor{red}{ 4.60} &\textcolor{red}{ 15.44} &\textcolor{red}{ 59.11} &\textcolor{red}{ 5.84} \\ \midrule
\multirow{2}{*}{GLM4v}  &36.49 &25.24 &26.24&19.66 &7.19 &27.93 &68.20 &2.64 \\
  &\textcolor{red}{ 31.56} &\textcolor{red}{19.00}&\textcolor{red}{ 24.00} &\textcolor{red}{ 18.86} &\textcolor{red}{ 5.56} &\textcolor{red}{ 30.50} &\textcolor{red}{ 75.37} &\textcolor{red}{ 2.71} \\ \midrule
\multirow{2}{*}{GPT-4o}  &70.24 &45.93 &47.42&31.68 &6.18 &25.31 &75.70 &3.38 \\
 &\textcolor{red}{ 60.65} &\textcolor{red}{33.05} &\textcolor{red}{ 49.57} &\textcolor{red}{ 31.60} &\textcolor{red}{ 6.05} &\textcolor{red}{ 27.97} &\textcolor{red}{ 77.16} &\textcolor{red}{ 3.32} \\ \midrule
\multirow{2}{*}{Qwen-vl-max}  &56.45 &27.42 &30.54&28.56 &4.93 &14.76 &46.47 &7.26 \\
  &\textcolor{red}{ 42.91} &\textcolor{red}{28.27}&\textcolor{red}{ 22.36} &\textcolor{red}{ 21.13} &\textcolor{red}{ 4.65} &\textcolor{red}{ 9.93} &\textcolor{red}{ 44.31} &\textcolor{red}{ 4.16} \\ \bottomrule
\end{tabular}}
\caption{The auto-metric evaluation result for the one-shot CoT in different doctor models. The black denotes the result is evaluated with the standard patient and the red denotes with the actor patient.}
\label{tab:auto-one-CoT}
\end{table*}

==> table/auto_zero_cot.tex <==
\begin{table*}[h]
\centering
\fontsize{9}{9}\selectfont{
\begin{tabular}{ccccc|c|ccc@{}}
\toprule
\multirow{2}{*}{Model} &\multicolumn{4}{c|}{Overall Competency} &Multi-turn &\multicolumn{3}{c}{Multi-modal} \\
  &Inquiry &Examination  &Diagnosis & Treatment &info\_gain &MMA &Contras-1 &Contras-2 \\ \midrule
\multirow{2}{*}{Gemini-pro}   &67.32 &21.70 &44.03&31.00 &4.02 &6.13 &39.77 &9.54 \\
&\textcolor{red}{ 62.50} &\textcolor{red}{25.56} &\textcolor{red}{ 45.87} &\textcolor{red}{ 30.75} &\textcolor{red}{ 3.40} &\textcolor{red}{ 9.09} &\textcolor{red}{ 54.86} &\textcolor{red}{ 10.04} \\ \midrule
\multirow{2}{*}{GLM4v}  &39.44 &18.31 &23.02&15.87 &4.59 &18.21 &59.77 &3.88 \\
  &\textcolor{red}{ 28.92} &\textcolor{red}{13.83}&\textcolor{red}{ 18.09} &\textcolor{red}{ 18.17} &\textcolor{red}{ 4.77} &\textcolor{red}{ 19.68} &\textcolor{red}{ 62.61} &\textcolor{red}{ 3.74} \\ \midrule
\multirow{2}{*}{GPT-4o}  &67.70 &34.44 &45.14&32.16 & 4.88 &18.21 &59.75 &3.75 \\
  &\textcolor{red}{ 60.91} &\textcolor{red}{35.18}&\textcolor{red}{ 44.44} &\textcolor{red}{ 30.09} &\textcolor{red}{ 4.43} &\textcolor{red}{ 9.01} &\textcolor{red}{ 25.67} &\textcolor{red}{ 1.59} \\ \midrule
\multirow{2}{*}{Qwen-vl-max} &53.68 &18.99 &25.56 &23.91 &4.21 &14.63 &64.31 &5.75 \\
  &\textcolor{red}{ 46.24} &\textcolor{red}{25.09}&\textcolor{red}{ 27.27} &\textcolor{red}{ 21.75} &\textcolor{red}{ 3.83} &\textcolor{red}{ 15.44} &\textcolor{red}{ 53.60} &\textcolor{red}{ 4.31} \\ \bottomrule
\end{tabular}}
\caption{The auto-metric evaluation result for the zero-shot CoT in different doctor models. The black denotes the result is evaluated with the standard patient and the red denotes with the actor patient.}
\label{tab:auto-zero-CoT}
\end{table*}

==> table/gender_bias.tex <==
\begin{table*}[h]
\centering
\fontsize{9}{9}\selectfont{
\begin{tabular}{ccccc|c|ccc}
\toprule
\multirow{2}{*}{Model} &\multicolumn{4}{c|}{Overall Competency} &Multi-turn &\multicolumn{3}{c}{Multi-modal} \\
  &Inquiry &Examination  &Diagnosis & Treatment &info\_gain &MMA &Contras-1 &Contras-2 \\ \midrule
\multirow{2}{*}{Gemini-pro}  &60.79 &34.59 &41.14&31.71 & 3.65 &11.50 &57.06 &12.10 \\
 &\textcolor{red}{ 60.70} &\textcolor{red}{27.27}&\textcolor{red}{ 38.51} &\textcolor{red}{ 27.49} &\textcolor{red}{ 4.03} &\textcolor{red}{ 8.61} &\textcolor{red}{ 48.94} &\textcolor{red}{ 6.47} \\ \midrule
\multirow{2}{*}{GPT-4o}  &59.75 &21.53 &35.40&25.86 &3.98 &14.16 &47.45 &2.79 \\
 &\textcolor{red}{ 59.97} &\textcolor{red}{30.40} &\textcolor{red}{ 40.65} &\textcolor{red}{ 31.59} &\textcolor{red}{ 4.76} &\textcolor{red}{ 14.82} &\textcolor{red}{ 45.99} &\textcolor{red}{ 2.18} \\ \midrule
\end{tabular}}
\caption{The auto-metric evaluation result for different genders in various doctor models. The black denotes the result is evaluated with the male patient case and the red denotes the female patient case.}
\label{tab:auto_gender}
\end{table*}


\begin{table*}[h]
\centering
\fontsize{9}{9}\selectfont{
\begin{tabular}{cccccc|c|ccc}
\toprule
\multirow{2}{*}{Model} &\multicolumn{5}{c|}{Overall Competency} &\multicolumn{1}{c|}{Multi-turn} &\multicolumn{3}{c}{Multi-modal} \\
\multicolumn{1}{c}{} &\multicolumn{1}{c}{Inquiry} &\multicolumn{1}{c}{Examination} &\multicolumn{1}{c}{Diagnosis} &\multicolumn{1}{c}{Treament}&\multicolumn{1}{c|}{C-K} &\multicolumn{1}{c|}{info\_gain} &\multicolumn{1}{c}{MMA} &\multicolumn{1}{c}{Contras-1} &\multicolumn{1}{c}{Contras-2} \\ \midrule
\multirow{2}{*}{Gemini-pro}  &3.12	&1.27&	3.35 &3.50	&3.27	&3.49  &2.50	&2.63	&3.00 \\
&\textcolor{red}{3.09}	&\textcolor{red}{1.12}&	\textcolor{red}{2.94}&	\textcolor{red}{3.25}&		\textcolor{red}{3.22}&		\textcolor{red}{3.42}&	  \textcolor{red}{2.27}&		\textcolor{red}{2.33}&		\textcolor{red}{2.5} \\ \midrule
\multirow{2}{*}{GPT-4o} &3.32	&1.64	&3.13	&3.43&3.56	&3.90  &2.73	&2.83	&2.40 \\
&\textcolor{red}{3.24}&	\textcolor{red}{1.79}&	\textcolor{red}{3.18}&	\textcolor{red}{3.71}&	\textcolor{red}{3.70}&	\textcolor{red}{4.01}& \textcolor{red}{2.40} &\textcolor{red}{2.45}&	\textcolor{red}{2.45} \\\midrule
\end{tabular}}
\caption{The LLM-based evaluation result for different genders in various doctor models. The black denotes the result is evaluated with the male patient case and the red denotes the female patient case.}
\label{tab:llm-gender}
\end{table*}

==> table/llm.tex <==
\begin{table*}[]
\centering
\fontsize{9}{9}\selectfont{
\begin{tabular}{@{}cccccc|c|ccc@{}}
\toprule
\multirow{2}*{Model} &\multicolumn{5}{c|}{Overall Competency} &Multi-turn &\multicolumn{3}{c}{Multi-modal} \\
 &Inquiry &Examination &Diagosis & Treatment &C-K &info\_gain &MMA &Contras-1 &Contras-2 \\ \midrule
\multirow{2}*{Mini-InternVL-1.5}  &2.52 &1.22 &2.11	&2.40 &2.86 &2.60 &1.78	&1.61	&1.85 \\
&\textcolor{red}{ 2.39} &\textcolor{red}{ 1.24} &\textcolor{red}{ 2.08} &\textcolor{red}{ 2.44}&\textcolor{red}{ 2.75} &\textcolor{red}{ 2.26}&\textcolor{red}{ 1.48} &\textcolor{red}{ 1.66} &\textcolor{red}{ 1.83} \\ \midrule
\multirow{2}*{InternVL-1.5} &2.49 &1.23 &2.01&2.48 &3.14 &2.67 &1.77 &1.82 &1.68 \\
 &\textcolor{red}{ 2.55} &\textcolor{red}{ 1.10} &\textcolor{red}{ 2.15} &\textcolor{red}{ 2.22} &\textcolor{red}{ 3.08} &\textcolor{red}{ 2.83} &\textcolor{red}{ 1.62} &\textcolor{red}{ 1.68} &\textcolor{red}{ 1.37} \\ \midrule
\multirow{2}*{Gemini-flash} &2.96 &1.35 &2.97&3.14 &3.51 &3.19 &2.29&2.63 &3.63 \\
 &\textcolor{red}{ 2.88} &\textcolor{red}{ 1.22} &\textcolor{red}{ 2.77}&\textcolor{red}{ 2.80} &\textcolor{red}{ 3.18} &\textcolor{red}{ 3.06} &\textcolor{red}{ 1.82} &\textcolor{red}{ 1.97} &\textcolor{red}{ 2.42} \\ \midrule
\multirow{2}*{Gemini-pro} &3.21 &1.42 &3.38	&3.65 &3.59 &3.75 &2.60 &2.67 &3.17 \\
 &\textcolor{red}{ 2.83} &\textcolor{red}{ 1.22} &\textcolor{red}{ 2.96} &\textcolor{red}{ 3.25}&\textcolor{red}{ 3.42} &\textcolor{red}{ 3.35} &\textcolor{red}{ 1.95} &\textcolor{red}{ 2.13} &\textcolor{red}{ 2.57} \\ \midrule
\multirow{2}*{GLM4v} &2.93 &1.25 &2.66 &2.90&3.51 &3.08 &2.34 &2.62 &2.88\\
 &\textcolor{red}{ 2.71} &\textcolor{red}{ 1.52} &\textcolor{red}{ 2.54} &\textcolor{red}{ 2.73}&\textcolor{red}{ 3.27} &\textcolor{red}{ 2.83} &\textcolor{red}{ 2.61} &\textcolor{red}{ 2.62} &\textcolor{red}{ 2.45} \\ \midrule
\multirow{2}*{GPT-4o} &3.63 &1.85 &3.62 &3.79&3.94 &4.12 &2.50 &2.58 &2.53 \\
 &\textcolor{red}{ 3.56} &\textcolor{red}{ 1.97} &\textcolor{red}{ 3.82} &\textcolor{red}{ 3.89}&\textcolor{red}{ 3.83} &\textcolor{red}{ 3.83} &\textcolor{red}{ 2.46} &\textcolor{red}{ 2.39} &\textcolor{red}{ 2.77} \\ \midrule
\multirow{2}*{GPT-4o mini} &3.49 &1.14 &3.36 &3.64&3.89 &3.79 &1.99 &1.59 &1.07 \\
 &\textcolor{red}{ 3.19} &\textcolor{red}{ 1.10} &\textcolor{red}{ 3.11} &\textcolor{red}{ 3.41}&\textcolor{red}{ 3.62} &\textcolor{red}{ 3.72} &\textcolor{red}{ 1.58} &\textcolor{red}{ 1.40} &\textcolor{red}{ 0.72} \\ \midrule
\multirow{2}*{GPT-4v} &3.71 &2.19 &3.77&3.59 &4.04 &4.31 &2.86 &3.08 &3.33 \\
 &\textcolor{red}{ 3.49} &\textcolor{red}{ 1.89} &\textcolor{red}{ 3.34} &\textcolor{red}{ 3.44} &\textcolor{red}{ 3.85} &\textcolor{red}{ 4.06} &\textcolor{red}{ 2.85} &\textcolor{red}{ 2.95} &\textcolor{red}{ 3.22} \\ \midrule
\multirow{2}*{Qwen-vl-chat-v1} &2.71 &1.03 &2.26 &2.45&2.89 &2.35 &1.68 &1.79 &1.68 \\
 &\textcolor{red}{ 2.32} &\textcolor{red}{ 1.08} &\textcolor{red}{ 2.30} &\textcolor{red}{ 2.73}&\textcolor{red}{ 2.36} &\textcolor{red}{ 2.22} &\textcolor{red}{ 1.60} &\textcolor{red}{ 1.76} &\textcolor{red}{ 1.60} \\ \midrule
\multirow{2}*{Qwen-vl-max} &2.96 &1.49 &2.66 &2.90&3.30 &3.27 &2.43 &2.61 &2.82 \\
 &\textcolor{red}{ 2.94} &\textcolor{red}{ 1.47} &\textcolor{red}{ 2.49} &\textcolor{red}{ 2.98}&\textcolor{red}{ 3.42} &\textcolor{red}{ 3.17} &\textcolor{red}{ 2.08} &\textcolor{red}{ 2.30} &\textcolor{red}{ 2.88} \\ \midrule
 \multirow{2}*{HuatuoGPT-Vision-7B} &22.41	&1.27	&1.94	&2.42	&2.79&	2.49&1.75	&1.67	&1.32 \\
 &\textcolor{red}{ 2.45} &\textcolor{red}{ 1.15} &\textcolor{red}{ 1.85} &\textcolor{red}{ 2.57}&\textcolor{red}{ 2.82} &\textcolor{red}{ 2.41} &\textcolor{red}{ 1.85} &\textcolor{red}{ 1.68} &\textcolor{red}{ 1.24} \\ \midrule
 \multirow{2}*{HuatuoGPT-Vision-34B} &2.85&	1.45	&2.28&	2.95&	3.25	&3.09&2.03	&1.87	&1.95 \\
 &\textcolor{red}{ 2.76} &\textcolor{red}{ 1.18} &\textcolor{red}{ 2.37} &\textcolor{red}{ 2.83}&\textcolor{red}{ 3.26} &\textcolor{red}{ 3.19} &\textcolor{red}{ 2.12} &\textcolor{red}{ 1.82} &\textcolor{red}{ 2.00} \\ \bottomrule
\end{tabular}}
\caption{The LLM-based evaluation result about the standard patient and actor patient of different doctor models. The black denotes the result is evaluated with the standard patient and the red denotes with the actor patient. The D\&T and C-K are the abbreviations of the diagnosis\&treatment and communication skill, respectively.}
\label{tab:llm}
\end{table*}

==> table/llm_one_cot.tex <==
\begin{table*}[h]
\centering
\fontsize{9}{9}\selectfont{
\begin{tabular}{cccccc|c|ccc}
\toprule
\multirow{2}{*}{Model} &\multicolumn{5}{c|}{Overall Competency} &\multicolumn{1}{c|}{Multi-turn} &\multicolumn{3}{c}{Multi-modal} \\
\multicolumn{1}{c}{} &\multicolumn{1}{c}{Inquiry} &\multicolumn{1}{c}{Examination} &\multicolumn{1}{c}{Diagnosis} &\multicolumn{1}{c}{Treatment}&\multicolumn{1}{c|}{C-K} &\multicolumn{1}{c|}{info\_gain} &\multicolumn{1}{c}{MMA} &\multicolumn{1}{c}{Contras-1} &\multicolumn{1}{c}{Contras-2} \\ \midrule
\multirow{2}{*}{Gemini-pro}  &2.48 &1.42 &2.60 &2.78&2.86 &2.30 &1.93 &2.25 &1.92 \\
&\textcolor{red}{ 2.30} &\textcolor{red}{ 1.37} &\textcolor{red}{ 2.77} &\textcolor{red}{ 2.83}&\textcolor{red}{ 2.71} &\textcolor{red}{ 2.28} &\textcolor{red}{ 2.12} &\textcolor{red}{ 2.32} &\textcolor{red}{ 2.43} \\ \midrule
\multirow{2}{*}{GLM4v} &2.98 &1.52 &2.93 &2.86&3.45 &3.23 &2.88 &3.03 &3.01 \\
 &\textcolor{red}{ 2.89} &\textcolor{red}{ 1.71} &\textcolor{red}{ 2.65} &\textcolor{red}{ 2.89} &\textcolor{red}{ 3.28} &\textcolor{red}{ 2.78} &\textcolor{red}{ 2.78} &\textcolor{red}{ 3.00} &\textcolor{red}{ 3.35} \\ \midrule
\multirow{2}{*}{GPT-4o} &3.69 &1.80 &3.67 &3.89&3.96 &4,32 &3.34 &3.52 &3.58 \\
 &\textcolor{red}{ 3.39} &\textcolor{red}{ 2.37} &\textcolor{red}{ 3.73} &\textcolor{red}{ 3.94}&\textcolor{red}{ 3.58} &\textcolor{red}{ 3.86} &\textcolor{red}{ 3.42} &\textcolor{red}{ 3.33} &\textcolor{red}{ 3.57} \\ \midrule
\multirow{2}{*}{Qwen-vl-max} &2.91 &1.27 &2.84 &2.94&3.21 &3.05 &1.78 &1.98 &2.22 \\
 &\textcolor{red}{ 2.93} &\textcolor{red}{ 1.53} &\textcolor{red}{ 2.33} &\textcolor{red}{ 2.52}&\textcolor{red}{ 2.98} &\textcolor{red}{ 2.69} &\textcolor{red}{ 1.80} &\textcolor{red}{ 1.82} &\textcolor{red}{ 2.14} \\ \bottomrule
\end{tabular}}
\caption{The LLM-based evaluation result for the one-shot CoT in different doctor models. The black denotes the result is evaluated with the standard patient and the red denotes with the actor patient.}
\label{tab:llm-one-CoT}
\end{table*}

==> table/llm_zero_cot.tex <==
\begin{table*}[h]
\centering
\fontsize{9}{9}\selectfont{
\begin{tabular}{cccccc|c|ccc}
\toprule
\multirow{2}{*}{Model} &\multicolumn{5}{c|}{Overall Competency} &\multicolumn{1}{c|}{Multi-turn} &\multicolumn{3}{c}{Multi-modal} \\
\multicolumn{1}{c}{} &\multicolumn{1}{c}{Inquiry} &\multicolumn{1}{c}{Examination} &\multicolumn{1}{c}{Diagnosis} &\multicolumn{1}{c}{Treatment}&\multicolumn{1}{c|}{C-K} &\multicolumn{1}{c|}{info\_gain} &\multicolumn{1}{c}{MMA} &\multicolumn{1}{c}{Contras-1} &\multicolumn{1}{c}{Contras-2} \\ \midrule

\multirow{2}*{Gemini-pro}  &3.30 &1.23 &3.28&3.44 &3.60 &3.93 &2.03 &2.32 &1.93 \\
&\textcolor{red}{ 2.97} &\textcolor{red}{ 1.13} &\textcolor{red}{ 3.04} &\textcolor{red}{ 3.36}&\textcolor{red}{ 3.47} &\textcolor{red}{ 3.56} &\textcolor{red}{ 2.37} &\textcolor{red}{ 2.57} &\textcolor{red}{ 2.93} \\ \midrule
\multirow{2}*{GLM4v} &2.65 &1.33 &2.22 &2.57&3.33 &3.02 &2.58 &2.77 &2.48 \\
 &\textcolor{red}{ 2.52} &\textcolor{red}{ 1.25} &\textcolor{red}{ 2.27}&\textcolor{red}{ 2.70}&\textcolor{red}{ 3.22} &\textcolor{red}{ 2.61} & \textcolor{red}{ 2.40} &\textcolor{red}{ 2.55} &\textcolor{red}{ 2.75} \\ \midrule
\multirow{2}*{GPT-4o} &3.51 &1.62 &3.24&3.55 &3.90 &3.96 &2.47 &2.53 &2.89 \\
 &\textcolor{red}{ 3.42} &\textcolor{red}{ 1.52} &\textcolor{red}{ 3.35} &\textcolor{red}{ 3.72}&\textcolor{red}{ 3.66} &\textcolor{red}{ 3.89} &\textcolor{red}{ 2.03} &\textcolor{red}{ 2.07} &\textcolor{red}{ 1.67} \\ \midrule
\multirow{2}*{Qwen-vl-max} &2.88 &1.23 &2.34  &2.74&3.40 &2.93 &2.15 &2.47 &2.68 \\
 &\textcolor{red}{ 2.83} &\textcolor{red}{ 1.28} &\textcolor{red}{ 2.35} &\textcolor{red}{ 2.82}&\textcolor{red}{ 3.20} &\textcolor{red}{ 2.79} &\textcolor{red}{ 2.05} &\textcolor{red}{ 2.09} &\textcolor{red}{ 2.32} \\ \bottomrule
\end{tabular}}
\caption{The LLM-based evaluation result for the zero-shot CoT in different doctor models. The black denotes the result is evaluated with the standard patient and the red denotes with the actor patient.}
\label{tab:llm-zero-CoT}
\end{table*}
